Metamorphic Testing for Web System Security

Security testing aims at verifying that the software meets its security properties. In modern Web systems, however, this often entails the verification of the outputs generated when exercising the system with a very large set of inputs. Full automation is thus required to lower costs and increase the effectiveness of security testing. Unfortunately, to achieve such automation, in addition to strategies for automatically deriving test inputs, we need to address the oracle problem, which refers to the challenge, given an input for a system, of distinguishing correct from incorrect behavior. In this paper, we propose Metamorphic Security Testing for Web-interactions (MST-wi), a metamorphic testing approach that integrates test input generation strategies inspired by mutational fuzzing and alleviates the oracle problem in security testing. It enables engineers to specify metamorphic relations (MRs) that capture many security properties of Web systems. To facilitate the specification of such MRs, we provide a domain-specific language accompanied by an Eclipse editor. MST-wi automatically collects the input data and transforms the MRs into executable Java code to automatically perform security testing. It automatically tests Web systems to detect vulnerabilities based on the relations and collected data. We provide a catalog of 76 system-agnostic MRs to automate security testing in Web systems. It covers 39% of the OWASP security testing activities not automated by state-of-the-art techniques; further, our MRs can automatically discover 102 different types of vulnerabilities, which correspond to 45% of the vulnerabilities due to violations of security design principles according to the MITRE CWE database. We also define guidelines that enable test engineers to improve the testability of the system under test with respect to our approach.

==> MR_example.tex <==
\section{A Practical Example}



==> catalog.tex <==
% !TEX root =  Main.tex
\section{A Catalog of Metamorphic Relations for Security Testing}

We have defined a catalog of Metamorphic Relations that enables automated security metamorphic testing.
We derived the catalog by considering the type of security test cases described in the OWASP security testing guidelines for Web applications. 
For each type of security test case we have identified one or more metamorphic relations that enables to determine the presence of the vulnerability targeted by the corresponding test case. 
If a metamorphic relation does not hold then the system is vulnerable.
Metamorphic relations capture high-level properties that generally hold on Web systems

 the presence of the vulnerability when it does not hold.
To build the metamorphic relation we have introduced a set of relational operators (functions) that capture common characteristics of Web and Android systems.







==> discussion.tex <==
% !TEX root =  Main.tex
\subsection{Reflections on Industrial Adoption}
\label{subsec:discussion}

Discussion...

==> tables/OWASPten.tex <==
% !TEX root =  ../Main.tex
\begin{table}[tb]
\footnotesize
\caption{Vulnerability types addressed by SMRL \MRs}
\begin{center}
\begin{tabular}{|p{7cm}|p{1cm}|}
\hline
\textbf{Vulnerability type}			&\textbf{\#MRs}\\
\hline
Injection				&0\\
Broken Authentication	&6\\
Sensitive Data Exposure	&5\\
XML External Entities	&0\\
Broken Access Control	&7\\
Security Misconfiguration	&3\\
Cross-site scripting		&0\\
Insecure Deserialization	&0\\
Using Vulnerable Components	&1\\
Insufficient Logging or Monitoring	&0\\
\hline
\end{tabular}
\end{center}
\label{default}
\end{table}%


==> tables/comboExampleCodeData.tex <==

\begin{figure*}[h!]
\begin{minipage}[b]{\textwidth}
\begin{minipage}[b]{10cm}
%\begin{figure}[tb]%[htbp]
%\begin{center}
%\vspace*{-0.8em}
%\includegraphics[width=8.5cm]{images/editorAuthz002HIDDEN}
\includegraphics[width=10cm]{images/BIG_generatedCode_AUTHZ_002_V3.PNG}
%\caption{A metamorphic relation to determine if the system is affected by bypass authorization schema vulnerabilities.}
%\vspace*{-1.9em}
\captionof{figure}{Java code for the metamorphic relation in Fig.~\ref{fig:mrExample}.}
%\caption{A metamorphic relation for the Bypass Authorization Schema vulnerability.}
%\vspace*{-0.8em}
\label{fig:mrExample}
%\end{center}
%\end{figure}
\end{minipage}
\hspace{5mm}
\begin{minipage}[b]{7cm}
\input{tables/grammar.tex}
\end{minipage}
\end{minipage}
\end{figure*}

==> tables/comboExamplePictureGrammar.tex <==

\begin{figure*}[h!]
\begin{minipage}[b]{\textwidth}
\begin{minipage}[b]{10cm}
%\begin{figure}[tb]%[htbp]
%\begin{center}
%\vspace*{-0.8em}
%\includegraphics[width=8.5cm]{images/editorAuthz002HIDDEN}
\includegraphics[width=10cm]{images/BIG_editorAuthz002V5.PNG}
%\caption{A metamorphic relation to determine if the system is affected by bypass authorization schema vulnerabilities.}
\tiny \emph{Note: package names had been partially blanked out for double-blind review.}
\vspace*{-2mm}
\captionof{figure}{A metamorphic relation for the Bypass Authorization Schema vulnerability.}
%\caption{A metamorphic relation for the Bypass Authorization Schema vulnerability.}
%\vspace*{-0.8em}
\label{fig:mrExample}
%\end{center}
%\end{figure}
\end{minipage}
\hspace{5mm}
\begin{minipage}[b]{7cm}
\input{tables/grammar.tex}
\end{minipage}
\end{minipage}
\end{figure*}

==> tables/grammar.tex <==
% !TEX root =  ../Main.tex

%\begin{table}[tb]
\scriptsize
%\vspace*{-1.0em}
%\scriptsize
%\caption{The grammar of \SMRL.}

%\vspace{-0.25cm}
%\begin{tabular}{| p{0.07cm} | p{7.8cm} |}
\begin{tabular}{|@{\hspace{0.1cm}}p{0.2cm} | @{\hspace{0.05cm}}p{6.5cm} |}
\LLRESET
%\LL & \textbf{import} static lu.svv.mr.language.Operations.*\manuallabel{fig:grammar:import}{\LINE}\\
\LL &\textbf{grammar} lang.SMRL \textbf{with} org.eclipse.xtext.xbase.Xbase\\
%\LL &\textbf{generate} sMRL "http://www.svv.lu/lang/SMRL"\\
\LL &\textbf{import} "http://www.eclipse.org/xtext/xbase/Xbase" \textbf{as} xbase
\vspace{1mm}\\ 
\LL &SMRL:\\
\LL &\hspace{2mm}    importSection=XImportSection?\manuallabel{fig:grammar:importSec}{\LINE}\\
\LL &\hspace{2mm}    elements+=AbstractElement*;\\
%\vspace{1mm}\\
\LL &AbstractElement:\\
\LL &\hspace{2mm}    PackageDeclaration $|$ MR;
\vspace{1mm}\\
\LL & PackageDeclaration:\manuallabel{fig:grammar:package}{\LINE}\\
\LL &\hspace{2mm}    `package` name=QualifiedName '\{' \\
\LL &\hspace{8mm}        elements+=AbstractElement*\\
\LL &\hspace{2mm}    '\}';
\vspace{1mm}\\ 
\LL &MR:\\
\LL &\hspace{2mm}    `MR` name=ValidID '\{'\manuallabel{fig:grammar:MRstart}{\LINE}\\
\LL &\hspace{8mm}        operations+=Operation\\
\LL &\hspace{2mm}    '\}';
\vspace{1mm}\\
\LL &Operation:\\
\LL &\hspace{2mm}   body=XBlockExpression;\manuallabel{fig:grammar:XEXPR}{\LINE}\\
\end{tabular}
\captionof{figure}{The \SMRL grammar.}
%\vspace*{-1.0em}
\label{tab:grammar}
%\end{table}%


==> tables/tableAUTHZ2.tex <==
\begin{table}[p]
\tiny
%\scriptsize
\caption{Metamorphic Relation in \SMRL for the Bypass Authorization Schema Vulnerability}
%\begin{tabular}{| p{0.07cm} | p{7.8cm} |}
\begin{tabular}{|@{\hspace{0.1cm}}p{0.2cm} | @{\hspace{0.05cm}}p{8.0cm} |}
\LLRESET
\LL & \textbf{import} static lu.svv.mr.language.Operations.*\\


package lu.svv.mr.owasp {

	MR OTG_AUTHZ_002 {
		{

			IMPLIES(
					equal ( Input(2), changeCredentials( Input(1), User() ) )
						&& cannotReachThroughGUI ( User(), Input(1) ),
					different(Output(Input(1)),Output(Input(2)) ) );
		
		}
	}

}

\end{tabular}
\end{center}
\label{default}
\end{table}%


==> tables/tableBinaryPatterns.tex <==


\begin{table}[]
\centering
\caption{Top-3 repeated patterns in MRs}
\label{tab:my-table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|clll}
\cline{1-2}  \\[0.1ex]
 Pattern & Number of repeats  &  &  &  \\[0.8ex] \cline{1-2} \\[0.1ex]
 [Precondition on action; Same user, Modify; Equal, Verify predicates] & 19 &  &  &  \\[0.8ex] \cline{1-2} \\[0.1ex]
[Precondition on user, Precondition on action; Same user, Modify; Different, Verify predicates]& 8 &  &  &  \\[0.8ex] \cline{1-2} \\[0.1ex]
 [Precondition on action; Same user, Add; Different] & 7  &  &  &  \\[0.8ex] \cline{1-2}
\end{tabular}%
}
\end{table}

==> tables/tableBooleanOperators.tex <==
% !TEX root =  ../Main.tex
\begin{table}[tb]
%\tiny
%\scriptsize
\footnotesize
\caption{Metamorphic expression operators.}
%\begin{tabular}{| p{0.07cm} | p{7.8cm} |}
%\vspace*{-1.2em}
\vspace{-0.25cm}
\begin{tabular}{|@{\hspace{0.1cm}}p{3cm} | @{\hspace{0.05cm}}p{1.0cm} |@{\hspace{0.05cm}}p{3.7cm} |}
\hline
\textbf{Operator}&\textbf{Truth}&\textbf{Java code generated}\\
&\textbf{value}&\textbf{by the SMRL compiler}\\
\hline
IMPLIES(boolean a, boolean b) & (!a)||b & if(a)\{ \\
&&\hspace{2mm}if(b)\{ /*property holds*/ \}\\
&&\hspace{2mm}else\{ return false; \}\\
&&\}\\
\hline
AND(boolean a, boolean b) & a\&\&b & if(a)\{ \}\\
&&\hspace{2mm} if(b)\{ /*property holds*/ \}\\
&&\hspace{2mm} else\{ return false; \}\\
&&else\{ return false; \}\\
\hline
OR(boolean a, boolean b) & a||b & if(a)\{ /*property holds*/ \}\\
&&else \{ if(b)\{ /*property holds*/ \}\\
&&\hspace{2mm} else\{ return false; \}\\
&&\}\\
\hline
FALSE(boolean a) & (!a) & if(a)\{ return false; \}\\
&&else \{ /*property holds*/ \}\\
\hline
NOT(boolean a) & (!a) & if(a)\{ return false; \}\\
&&else \{ /*property holds*/ \}\\
\hline
TRUE(boolean a) & a & if(a)\{ /*property holds*/ \}\\
&&else \{ return false; \}\\
\hline
EQUAL(Object a,Object b) & a == b& if( alreadyUsed(a) )\\
&&\hspace{2mm} return a.equals(b); \\
&&else \{ dataProvider.set(a,b.clone()); \\
&&\hspace{2mm} return true; \}\\
\hline
\end{tabular}
%\vspace*{-1.6em}
\label{table:booleanOperators}
\end{table}%


==> tables/tableCrawling.tex <==
% !TEX root =  ../Main.tex
\begin{table}[tb]
%\tiny
%\scriptsize
\footnotesize
\caption{Summary of RQ2 results.}
%\vspace{-0.25cm}
\begin{tabular}{|@{\hspace{0.1cm}}p{1.5cm} | @{\hspace{0.05cm}}p{2.0cm} | @{\hspace{0.05cm}}p{5mm} | @{\hspace{0.05cm}}p{5mm} | @{\hspace{0.05cm}}p{5mm} |  @{\hspace{0.05cm}}p{10mm} | @{\hspace{0.05cm}}p{5mm} |  }
\hline
\textbf{Case study}&\textbf{User Roles}&\textbf{Crawljax graphs}\\
\textbf{Case study}&\textbf{User Roles}&\textbf{Total Nodes}&\textbf{Total edges}\\
\hline
\IWS	& 4 & 4& 0& 0 & 1.0 & 1.0\\
\hline
Jenkins 2.121.1	& 9 \cite{JV1,JV2,JV3,JV4,JV5,JV6,JV7,JV8,JV9}& \multirow{2}{*}{10} & \multirow{2}{*}{0} &   \multirow{2}{*}{1}  &   \multirow{2}{*}{1.0} & \multirow{2}{*}{0.91}   \\
Jenkins 2.12& 2 \cite{JV10,JV11}& & & & &\\
\hline
\end{tabular}
%\vspace{-0.5cm}
\label{table:resultsRQ2}
\end{table}%


%\begin{table}[tb]
%%\tiny
%%\scriptsize
%\footnotesize
%\caption{Oracle problem in OWASP testing activities.}
%%\begin{tabular}{| p{0.07cm} | p{7.8cm} |}
%%\vspace*{-1.2em}
%\begin{tabular}{|c | @{\hspace{0.1cm}}p{3cm} | @{\hspace{0.05cm}}p{1.0cm} |}
%\hline
%&\textbf{Oracle automation strategy}\\
%\hline
%\textbf{Testing activities not }
%&Not required	 &16\\
%\textbf{affected by the oracle} 
%&Single assertion &	9\\
%\textbf{problem.}
%&Implicit oracle	& 4\\
%&Catalog-based	& 11\\
%\hline
%\textbf{Testing activities affected }
%&Manual	& 13\\
%\textbf{by the oracle  problem.}
%&Dedicated methods	& 27\\
%&Metamorphic testing & 17\\
%%TOTAL & 99\\
%\hline
%\end{tabular}
%\vspace*{-1.2em}
%\label{table:OWASPtestingActivities}
%\end{table}%


==> tables/tableMRcatalog.tex <==
% !TEX root =  ../Main.tex
\begin{table*}[tb]
%\tiny
\scriptsize
\caption{Excerpt of the metamorphic relation catalog for security testing.} 
%For each OWASP testing activity, we report one metamorphic relation only.}
%\begin{tabular}{| p{0.07cm} | p{7.8cm} |}
\vspace*{-1.6em}
\begin{tabular}{@{\hspace{0.1cm}}p{8.4cm} @{\hspace{0.1cm}}p{8.4cm} }
\begin{tabular}{|p{8cm}|}
%\hline
%\textbf{OWASP testing activity with corresponding MR.}\\
\hline
\textbf{OTG-AUTHN-001}: Testing for Credentials Transported over an Encrypted Channel
\\
%height = 0.2*num of lines	
\includegraphics[height=1.2cm]{images/OTG_AUTHN_001.PNG}
\\
\emph{Description}: The login interface should not be displayed on the http channel.	
\\
\hline
\textbf{OTG-AUTHN-004}: Testing for bypassing authentication schema
\\	
\includegraphics[height=1.4cm]{images/OTG_AUTHN_004.PNG}
\\
\emph{Description}: Without begin authenticated, a user should not be able to access a page that normally can be reached only through the user interface of authenticated users.
\\

\hline
\textbf{OTG-AUTHN-010}: Testing for Weaker authentication in alternative channel
\\	
\includegraphics[height=1.2cm]{images/OTG_AUTHN_010.PNG}
\\
\emph{Description}: Without begin authenticated, a user should not be able to access a page that normally can be reached only through the user interface of authenticated users, even if he tries on the http channel.
\\

\hline
\textbf{OTG-AUTHZ-001}: Testing Directory traversal/file include
\\	
\includegraphics[height=1.6cm]{images/OTG_AUTHZ_001.png}
\\
\emph{Description}: A file path passed in a parameter should never enable a user to access data that is not provided by the user interface.	
\\

%\hline
%\textbf{OTG-AUTHZ-002}: Testing for bypassing authorization schema
%\\
%\includegraphics[height=1.4cm]{images/OTG_AUTHZ_002_01b.png}
%\\
%\emph{Description}: A URL that cannot be reached by a user while navigating the user interface should not be available to that same user even when she directly requests the URL to the server. For this reason, an input sequence that is valid for a given user, should not lead to the same output when it is executed by another user, if it includes access to a URL with these characteristics.	
%\\

\hline
\textbf{OTG-AUTHZ-003}: Testing for Privilege Escalation
\\	
\includegraphics[height=1.8cm]{images/OTG_AUTHZ_003.png}
\\
\emph{Description}: A user should not succeed in performing an operation on behalf of another user by simply replacing the user id passed as parameter in the URL.
\\
\hline

\textbf{OTG-AUTHZ-004}: Testing for Insecure Direct Object References
\\	
\includegraphics[height=1.8cm]{images/OTG_AUTHZ_004.png}
\\
\emph{Description}: A random value passed in a parameter should never enable a user to access data that is not provided already by the user interface (i.e., the system should return either data that can be accessed from the user interface or an error).	
\\
\hline




\textbf{OTG-BUSLOGIC-005}: Test Number of Times a Function Can be Used
\\	
\includegraphics[height=1.4cm]{images/OTG_BUSLOGIC_005.png}
\\
\emph{Description}:  If the URL of an action (e.g., the URL of the POST request sent when clicking on a \emph{reset password} button) changes over different executions of a same input sequence, then that URL is likely to be disposable and thus it is not expected to return the same result if accessed twice.
%\hline
\\
\hline




\end{tabular}
&
\begin{tabular}{|p{8.4cm}|}
\hline
\textbf{OTG-CONFIG-007}: Test HTTP Strict Transport Security
\\	
\includegraphics[height=1.6cm]{images/OTG_CONFIG_007.PNG}
\\
\emph{Description}:  In the presence of HTTP Strict Transport Security header, the browser should automatically be redirected to use the HTTPS channel and the system should return the expected page.
\\
\hline
\textbf{OTG-CRYPST-004}: Testing for Weak Encryption
\\	
\includegraphics[height=1.2cm]{images/OTG_CRYPST_004.PNG}
\\
\emph{Description}:  The system should prevent the use of weak encryption protocol. For this reason, when an encrypted channel is in use, the enforcement of a weak encryption protocol should never let a user access the requested data.
\\
%\hline
%\textbf{OTG-IDENT-003}: Test Account Provisioning Process
%\\	
%\includegraphics[height=1.4cm]{images/OTG_IDENT_003.PNG}
%\\
%\emph{Description}:  On Web systems, e-mails are typically used to confirm accounts or reset passwords. For this reason, for any input sequence that involve reading an e-mail, if the email contains a URL which appears to be a disposable one, then the same URL should not be accessible twice, otherwise we may have a problem in the account provisioning process.
%\\

\hline
\textbf{OTG-INPVAL-003}: Testing for HTTP Verb Tampering
\\	
\includegraphics[height=1.2cm]{images/OTG_INPVAL_003.png}
\\
\emph{Description}:  Accessing a URL with different methods (e.g., GET and UPDATE) should lead to different results.
\\
\hline
\textbf{OTG-INPVAL-004}: Testing for HTTP Parameter pollution
\\	
\includegraphics[height=1.6cm]{images/OTG_INPVAL_004.png}
\\
\emph{Description}:  In the presence of duplicated parameters, results should not change.
\\

\hline
\textbf{OTG-SESS-003}: Testing for Session Fixation
\\	
\includegraphics[height=1.2cm]{images/OTG_SESS_003_01.png}
\\
\emph{Description}:  A login action performed by a user already authenticated should always trigger the generation of a new session ID.
\\
%\hline
\\
\hline
\textbf{OTG-SESS-007}: Test Session Timeout
\\	
\includegraphics[height=1.4cm]{images/OTG_SESS_007.png}
\\
\emph{Description}:  An action that requires authentication should never lead to the expected output if executed after the session timeout (e.g., a login screen is expected).
\\
\hline
\textbf{OTG-SESS-008}: Testing for Session puzzling
\\	
\includegraphics[height=1.2cm]{images/OTG_SESS_008.png}
\\
\emph{Description}:  An action that does not require authentication should never enable an unauthenticated user to execute a follow-up action that requires authentication.
\\
\hline

\textbf{OTG-SESS-006}: Testing for logout functionality
\\	
\includegraphics[height=1.2cm]{images/OTG_SESS_003_01.png}
\\
\emph{Description}:  Any action following a logout should trigger the generation of a new session ID.
\\
\hline


\end{tabular}




%\hline
\end{tabular}
\vspace*{-1.4em}
\label{table:MRcatalog}
\end{table*}%


==> tables/tableMRcatalogShort.tex <==
% !TEX root =  ../Main.tex
\begin{table*}[h]
%\tiny
\scriptsize
\caption{Excerpt of our \MRs catalog for security testing.}

%For each OWASP testing activity, we report one metamorphic relation only.}
%\begin{tabular}{| p{0.07cm} | p{7.8cm} |}
%\vspace*{-1.6em}
%\begin{tabular}{@{\hspace{0.1cm}}p{8.4cm} @{\hspace{0.1cm}}p{8.4cm} }
\begin{tabular}{|@{\hspace{1mm}}p{10.2cm}|@{\hspace{1mm}}p{7.2cm}@{\hspace{0mm}}|}
%\caption{Excerpt of our \MRs catalog for security testing.}
%\hline
%\textbf{OWASP testing activity with corresponding MR.}\\
\hline
\textbf{OTG-AUTHN-001}: Testing for credentials transported over an encrypted channel &
\emph{Description}: A login operation should not succeed if performed on the http channel. The 1st parameter of the operator \texttt{IMPLIES} is a
\\
\begin{minipage}{10cm}
\vspace{-1mm}
\includegraphics[height=2.75cm]{images/BIG_OTG_AUTHN_001_.PNG} 
\end{minipage}
&
\begin{minipage}{7.2cm}
  boolean expression with three clauses joined with logical conjunctions. The 1st clause checks if the current action performs a login. The 2nd clause defines the follow-up input. The 3rd clause changes the channel of the login action in the follow-up input. 
The 2nd parameter of IMPLIES checks if the output generated by the login operation is different in the two cases.
\vspace{9mm}
\end{minipage}
\\
%\hline
%\textbf{OTG-AUTHN-004}: Testing for bypassing authentication schema &\emph{Description}: Without being authenticated, a user should not be
%\\
%\begin{minipage}{10cm}	
%\includegraphics[height=2.8cm]{images/BIG_OTG_AUTHN_004.PNG} 
%\end{minipage}
%
%&\begin{minipage}{6.5cm}
%able to access a page that normally can be reached only through the user interface of authenticated users. 
%The 1st parameter of the operator \texttt{IMPLIES}	is a boolean expression with three clauses joined with logical conjunction.
%The 1st clause checks if the current action has been performed after a login. 
%The 2nd clause checks if the current action has ever been performed by a non authenticated user.
%The 3rd clause defines a follow-up input that performs only the given action, without logging-in before. 
%The 2nd parameter of IMPLIES checks if the output generated by the action is different in the two cases.
%\end{minipage}
%\\
%\hline
%\textbf{OTG-AUTHN-010}: Testing for Weaker authentication in alternative channel
%\\
%\begin{minipage}{10cm}	
%\includegraphics[height=2.8cm]{images/BIG_OTG_AUTHN_010.PNG}
%\end{minipage}	
%&\emph{Description}: Without begin authenticated, a user should not be able to access a page that normally can be reached only through the user interface of authenticated users, even if he tries on the http channel.
%\\
%\hline
%\textbf{OTG-SESS-003}: Testing for session fixation&
%\\	
%\begin{minipage}{10cm}
%\includegraphics[height=2.8cm]{images/BIG_OTG_SESS_003.png}
%\end{minipage}
%& 
%\begin{minipage}{5cm}
%\emph{Description}:  A login action performed by a user already authenticated should always trigger the generation of a new session ID.
%This metamorphic relation contains two nested loops; the first iterates over the inputs to find a login action, the second iterates over the actions that follow the login.
%The second loop is necessary to check that the the login repeated at any point of the action sequence lead to a new session ID.
%The 1st parameter of the operator \texttt{IMPLIES}	is a boolean expression with two clauses joined with logical conjunction.
%The 1st clause checks if the current action is a login operation. 
%The 2nd clause defines a follow-up input with the login action being duplicated in a certain position.
%The 2nd parameter of IMPLIES checks if the session ID of the response page sent after the two successive login actions is different.
%\end{minipage}
%\\
\hline
\textbf{OTG-AUTHZ-001}: Testing for directory traversal/file include&\emph{Description}: A file path passed in a parameter should never enable a user to access data that is not provided by the user interface. 
\\	
\begin{minipage}{10cm}
\includegraphics[height=3.6cm]{images/BIG_OTG_AUTHZ_001.png}
\end{minipage}
&
\begin{minipage}{7.2cm}
This metamorphic relation contains two nested loops; the first iterates over the actions in the input sequence, the second iterates over the parameters of the action.
The 1st parameter of the operator \texttt{IMPLIES}	is a boolean expression with two clauses joined with a logical conjunction.
The 1st clause defines a follow-up input that is a copy of the source input.
The 2nd clause set the value of a parameter to a random file path.
The 2nd parameter of IMPLIES verifies the result. It is implemented as an OR operation where the 1st parameter verifies that the follow-up input leads to an error page. 
The 2nd parameter deals with the case in which the generated request is valid, and verifies that the returned content is something that the user has the right to access.
The framework evaluates the \MR as many times as needed to provide 100 different random file paths to the parameters of the action in the position \TEXTTT{pos}.
%\vspace{3mm}
\end{minipage}	
\\
\hline
\textbf{OTG-SESS-003}: Testing for session fixation&\emph{Description}: A signup action should always lead to a new session ID, even when performed by a user who is already logged-in. This\\	
\begin{minipage}{10cm}
\includegraphics[height=3.4cm]{images/BIG_OTG_SESS_003_02_.png}
\end{minipage}
&
\begin{minipage}{7.2cm}
 metamorphic relation contains two nested loops iterating over the actions of two distinct source input sequences (i.e., \texttt{Input(1)} and \texttt{Input(2)} ). The first loop looks for a signup action (i.e., `signup'), the second looks for an action (i.e., `f') following a login.
The 1st parameter of the operator \texttt{IMPLIES}	is a boolean expression with three clauses joined with a logical conjunction.
The 1st clause checks if we are in the presence of a signup action.
The 2nd clause checks if the action `f' follows a login. 
The 3rd clause defines a follow-up input by copying the signup action after the action `f' in the source input \texttt{Input(2)}.
The 2nd parameter of IMPLIES verifies the result by checking that the session ID following the signup action is different than the one of the previous page.
\vspace{1mm}
\end{minipage}	
\\
\hline
\textbf{CWE\_302\_471\_472\_784\_807}: Testing for assumed-immutable elements&\emph{Description}: Altering a boolean value in a session cookie should \\
\begin{minipage}{10cm}
\includegraphics[width=9.5cm]{images/CWE_302_471_472_784_807.png}
\end{minipage}
&
\begin{minipage}{7.2cm}
not enable an attacker to perform actions he is not authorized to. This MR creates a follow-up input where a follow-up user performs the actions in the source input.
The MR creates a new follow-up input for every session cookie that might be altered (8).
  When iterating over the list of cookies to alter, the MR verifies that the URL was not tested before (10),
  the value set in the session cookie is a boolean (11),
  the URL should not be accessed by the follow-up user (12), the output obtained for the source and follow-up inputs are different (13). If the outputs obtained for the source and follow-up inputs are not different  we are in the presence of another vulnerability (i.e., \emph{OTG\_AUTHZ\_002}). The MR then creates a second follow-up input (14), it copies the session cookie obtained for the first follow-up input (15), and then flips the boolean values in it (16). After flipping the values, the output of the second follow-up input should not become equal to the output of the source input (e.g., because of setting a cookie as \texttt{administrator=true}) or an error should be reported.
  \vspace{5mm}
\end{minipage}	
\\
\hline
%\end{xtabular*}
\end{tabular}
\label{table:MRcatalog}
\end{table*}


\begin{table*}[h]
%\tiny
\scriptsize
\caption{Excerpt of our \MRs catalog for security testing (part 2).} 
%For each OWASP testing activity, we report one metamorphic relation only.}
%\begin{tabular}{| p{0.07cm} | p{7.8cm} |}
%\vspace*{-1.6em}
%\begin{tabular}{@{\hspace{0.1cm}}p{8.4cm} @{\hspace{0.1cm}}p{8.4cm} }
\begin{tabular}{|@{\hspace{1mm}}p{10.2cm}|@{\hspace{1mm}}p{7.2cm}@{\hspace{0mm}}|}

\textbf{CWE\_15\_639\_OTG\_AUTHZ\_004}: Testing for externally controlled elements&\emph{Description}: Replacing a parameter value with a value used by another user \\
\begin{minipage}{10cm}
\includegraphics[height=4cm]{images/CWE_15_639_OTG_AUTHZ_004.png}
\end{minipage}
&
\begin{minipage}{7.2cm}
should not enable an attacker to collect data she is not authorized to. This MR creates a follow-up input where a the user performs the actions in the source input except for one parameter that is replaced with a value that has been observed only with other users (e.g., their ID).

  \vspace{5mm}
\end{minipage}	
\\

\hline
\textbf{OTG\_AUTHZ\_002c}: Testing for incorrect user management &\emph{Description}: A URL that cannot be reached by a user while navi-  \\
\begin{minipage}{10cm}
\includegraphics[height=4.5cm]{images/OTG_AUTHZ_002c.png}
\end{minipage}
&
\begin{minipage}{7.2cm}
gating the user interface should not be available to that same user, even when she directly requests the URL to the server. This MR creates a follow-up input that directly requests the action-y from the sequence of actions accessible if the user is authenticated (i.e. the action-y is performed after the login).
  \vspace{5mm}
\end{minipage}	
\\
\hline



%\multicolumn{2}{l}{\hspace{-2mm}\begin{minipage}{17.7cm}
%\vspace{2mm}

\textbf{CWE\_613}: Testing for insufficient session expiration &\emph{Description}: A logout action should always lead to a new session. \\
\begin{minipage}{10cm}
\includegraphics[height=4.5cm]{images/CWE_613.png}
\end{minipage}
&
\begin{minipage}{7.2cm}
This MR contains two nested loops to iterate over all actions. The first loop iterates over all the actions to find a logout action, named action-x.The second loop iterates over all the actions to find an action performed after the login, named action-y. The MR defines a follow-up input that tries to perform action-y without any authentication step. The session is not expired if the session ID is the same after and before the logout.
  \vspace{5mm}
\end{minipage}	
\\
\hline


%% CWE_814 should be added 



\end{tabular}
\label{table:MRcatalog2}
%\vspace*{-1.4em}
\end{table*}




\begin{table*}[tb]
%\tiny
\scriptsize
\caption{Excerpt of our \MRs catalog for security testing (part 3).} 
%For each OWASP testing activity, we report one metamorphic relation only.}
%\begin{tabular}{| p{0.07cm} | p{7.8cm} |}
%\vspace*{-1.6em}
%\begin{tabular}{@{\hspace{0.1cm}}p{8.4cm} @{\hspace{0.1cm}}p{8.4cm} }
\begin{tabular}{|@{\hspace{1mm}}p{10.2cm}|@{\hspace{1mm}}p{7.2cm}@{\hspace{0mm}}|}

\textbf{CWE\_841}: Testing for improper enforcement of behavioral workflow
&\emph{Description}: The software supports a session in which an actor       \\
\begin{minipage}{10cm}
\includegraphics[height=4.5cm]{images/CWE_841.png}
\end{minipage}
&
\begin{minipage}{7.2cm}
 must perform more than one behaviour, but it does not properly ensure that the actor performs the behaviours in the required sequence. This MR reverses the sequence of actions that requires the user to be authenticated before taking it. Consider a sequence of actions for creating an account on a website, which requires the user to verify the email address before having an active account. The action sequence includes signing up, email verification, and logging in. In this MR, we changed the sequence of actions that skipped the email verification step. The MR contains two nested for loops to iterate over all actions. The first loop iterates over all the actions to find a signup action. The second loop iterates over all the actions to find a login action performed after the signup. The follow-up input will perform the login exactly after the signup action. It is expected that the system gives two different outputs or will give an error by executing the follow-up input.
  \vspace{5mm}
\end{minipage}	
\\
\hline


\textbf{CWE\_79\_a\_XSSreflected}: Testing for reflected cross-site scripting &\emph{Description}: The software does not neutralize or incorrectly neu-\\
\begin{minipage}{10cm}
\includegraphics[height=6cm]{images/CWE_79a_XSSreflected.png}
\end{minipage}
&
\begin{minipage}{7.2cm}
tralizes user-controllable input before it is placed in output that is used as a web page that is served to other users. This MR, includes two nested for loops that iterate over all parameters of the action to inject a XSS string as the value of the parameter.
To speed  of the process, it checks if the parameter of the action URL has not seen before, and verifies that the action does not originally contain any alert.
The MR Creates the follow-up input by copying the Input(1), and setting the injected XSS string as the parameter value of the follow-up input.
It is expected that either the system neutralize the effect of the injected value, or the attack was not performed.
  \vspace{5mm}
\end{minipage}	
\\
\hline


\textbf{CWE\_94\_96\_b}: Testing for static code injection &\emph{Description}: The software receives input from an upstream comp-\\
\begin{minipage}{10cm}
\includegraphics[height=6.95cm]{images/CWE_94_96_b.png}
\end{minipage}
&
\begin{minipage}{7.2cm}
onent, but it does not neutralize or incorrectly neutralizes code syntax before inserting the input into an executable resource, such as a library, configuration file, or template.  This MR contains two nested for loops to iterate over all input entries. in (5), it makes sure the user will submit the form
 This MR tries to inject some malformed strings(static code) into all input entries of the follow-up input. It is expected
 from the system to show an error message or content that the follow-up user already has the right to access.
  \vspace{5mm}
\end{minipage}	
\\
\hline




\end{tabular}
\label{table:MRcatalog3}
%\vspace*{-1.4em}
\end{table*}




\begin{table*}[tb]
%\tiny
\scriptsize
\caption{Excerpt of our \MRs catalog for security testing (part 4).}

%For each OWASP testing activity, we report one metamorphic relation only.}
%\begin{tabular}{| p{0.07cm} | p{7.8cm} |}
%\vspace*{-1.6em}
%\begin{tabular}{@{\hspace{0.1cm}}p{8.4cm} @{\hspace{0.1cm}}p{8.4cm} }
\begin{tabular}{|@{\hspace{1mm}}p{10.2cm}|@{\hspace{1mm}}p{7.2cm}@{\hspace{0mm}}|}

\textbf{CWE\_792\_793\_794\_795\_796\_797\_A}: Testing for incomplete filtering of one or more instances of special elements
&\emph{Description}: The software receives data from an upstream comp-\\
\begin{minipage}{10cm}
\includegraphics[height=4.5cm]{images/CWE_792_A.png}
\end{minipage}
&
\begin{minipage}{7.2cm}
onent, but only accounts for special elements positioned relative to a marker (e.g. "at the beginning/end of a string; the second argument"), thereby missing remaining special elements that may exist before sending it to a downstream component. We have implemented different variations of this MR that insert the spacial character in different positions of the input string. This MR contains two nested loops that iterate the overall parameters of the actions. It inserts the special element at the beginning of the input value. It is expected that the system will show an error page or neutralize the input. 
  \vspace{5mm}
\end{minipage}	
\\
\hline






\end{tabular}
\label{table:MRcatalog3}
%\vspace*{-1.4em}
\end{table*}

==> tables/tableOWASPTestingActivities.tex <==
% !TEX root =  ../Main.tex
%\begin{table}[tb]
%%\tiny
%%\scriptsize
%\footnotesize
%\caption{Oracle automation strategies for security testing.}
%%\vspace{-0.25cm}
%\begin{tabular}{|@{\hspace{0.1cm}}p{4cm} | @{\hspace{0.05cm}}p{4.0cm} |}
%\hline
%\textbf{Oracle automation strategy}&\textbf{\# OWASP activities automated}\\
%\hline
%Implicit oracle	& 2\\
%Catalog-based	& 6\\
%No oracle needed	 &19\\
%Manual oracle	& 25\\
%Vulnerability-specific approaches	& 22\\
%Metamorphic testing & 16\\
%%TOTAL & 99\\
%\hline
%\end{tabular}
%%\vspace{-0.5cm}
%\label{table:OWASPtestingActivities}
%\end{table}%
%
\begin{table}[tb]
\scriptsize
\begin{minipage}[t]{4.35cm}
\caption{Oracle automation strategies for security testing*}
%\vspace{-0.25cm}
\begin{tabular}{|@{\hspace{0.05cm}}p{2.4cm} | @{\hspace{0.05cm}}p{1.3cm}|}
\hline
\textbf{Oracle automation strategy}&\textbf{\# OWASP activities automated}\\
\hline
Implicit oracle	& 2\\
Catalog-based	& 6\\
No oracle needed	 &19\\
Manual oracle	& 25\\
Vulnerability-specific & 22\\
Metamorphic testing & 16\\
%TOTAL & 99\\
\hline
\end{tabular}
\label{table:OWASPtestingActivities}
\vspace{0.1cm}
\footnotesize{*Details are available online~\cite{WebSMRL}.}
\end{minipage}
\begin{minipage}[t]{4.4cm}
\caption{Vulnerability types addressed by SMRL \MRs*}
\begin{tabular}{|@{\hspace{0.05cm}}p{3.3cm}|@{\hspace{0.05cm}}p{6mm}|}
\hline
\textbf{Vulnerability type}			&\textbf{\#MRs}\\
\hline
Injection				&0\\
Broken Authentication	&6\\
Sensitive Data Exposure	&5\\
XML External Entities(XEE)&0\\
Broken Access Control	&7\\
Security Misconfiguration	&3\\
Cross-site scripting	(XSS)	&0\\
Insecure Deserialization	&0\\
Vulnerable Components	&1\\
Insufficient Logging	&0\\
\hline
\end{tabular}
\label{table:OWASP10}
\end{minipage}
\end{table}%


==> tables/tableOWASPTestingActivitiesCategories.tex <==
% !TEX root =  ../Main.tex
\begin{table}[tb]
%\tiny
\tiny
\caption{OWASP testing activities.}
%\begin{tabular}{| p{0.07cm} | p{7.8cm} |}

\begin{tabular}{|@{\hspace{0.1cm}}p{2cm} | @{\hspace{0.05cm}}p{6.0cm} |}
\hline
\textbf{Data method}&\textbf{Description}\\
\hline
OTG-INFO-001& Conduct Search Engine Discovery and Reconnaissance for Information Leakage \\
OTG-INFO-002& Fingerprint Web Server \\
OTG-INFO-003& Review Webserver Metafiles for Information Leakage \\
OTG-INFO-004& Enumerate Applications on Webserver \\
OTG-INFO-005& Review Webpage Comments and Metadata for Information Leakage \\
OTG-INFO-006& Identify application entry points \\
OTG-INFO-007& Map execution paths through application \\
OTG-INFO-008& Fingerprint Web Application Framework \\
OTG-INFO-009& Fingerprint Web Application \\
OTG-INFO-010& Map Application Architecture \\
OTG-CONFIG-001& Test Network/Infrastructure Configuration \\
OTG-CONFIG-002& Test Application Platform Configuration \\
OTG-CONFIG-003& Test File Extensions Handling for Sensitive Information \\
OTG-CONFIG-004& Review Old, Backup and Unreferenced Files for Sensitive Information \\
OTG-CONFIG-005& Enumerate Infrastructure and Application Admin Interfaces \\
OTG-CONFIG-006& Test HTTP Methods \\
OTG-CONFIG-007& Test HTTP Strict Transport Security \\
OTG-CONFIG-008& Test RIA cross domain policy \\
OTG-CONFIG-009& Test File Permission \\
OTG-IDENT-001& Test Role Definitions \\
OTG-IDENT-002& Test User Registration Process \\
OTG-IDENT-003& Test Account Provisioning Process \\
OTG-IDENT-004& Testing for Account Enumeration and Guessable User Account \\
OTG-IDENT-005& Testing for Weak or unenforced username policy \\
OTG-AUTHN-001& Testing for Credentials Transported over an Encrypted Channel \\
OTG-AUTHN-002& Testing for default credentials \\
OTG-AUTHN-003& Testing for Weak lock out mechanism \\
OTG-AUTHN-004& Testing for bypassing authentication schema \\
OTG-AUTHN-005& Test remember password functionality \\
OTG-AUTHN-006& Testing for Browser cache weakness \\
OTG-AUTHN-007& Testing for Weak password policy \\
OTG-AUTHN-008& Testing for Weak security question/answer \\
OTG-AUTHN-009& Testing for weak password change or reset functionalities \\
OTG-AUTHN-010& Testing for Weaker authentication in alternative channel \\
OTG-AUTHZ-001& Testing Directory traversal/file include \\
OTG-AUTHZ-002& Testing for bypassing authorization schema \\
OTG-AUTHZ-003& Testing for Privilege Escalation \\
OTG-AUTHZ-004& Testing for Insecure Direct Object References \\
OTG-SESS-001& Testing for Bypassing Session Management Schema \\
OTG-SESS-002& Testing for Cookies attributes \\
OTG-SESS-003& Testing for Session Fixation \\
OTG-SESS-004& Testing for Exposed Session Variables \\
CSRF & Testing for Cross Site Request Forgery \\
OTG-SESS-006& Testing for logout functionality \\
OTG-SESS-007& Test Session Timeout \\
OTG-SESS-008& Testing for Session puzzling \\
OTG-INPVAL-001& Testing for Reflected Cross Site Scripting \\
OTG-INPVAL-002& Testing for Stored Cross Site Scripting \\
OTG-INPVAL-003& Testing for HTTP Verb Tampering \\
OTG-INPVAL-004& Testing for HTTP Parameter pollution \\
OTG-INPVAL-005& Testing for SQL Injection \\

OTG-INPVAL-006& Testing for LDAP Injection \\
OTG-INPVAL-007& Testing for ORM Injection \\
OTG-INPVAL-008& Testing for XML Injection \\
OTG-INPVAL-009& Testing for SSI Injection \\
OTG-INPVAL-010& Testing for XPath Injection \\
OTG-INPVAL-011& IMAP/SMTP Injection \\
OTG-INPVAL-012& Testing for Code Injection \\

OTG-INPVAL-013& Testing for Command Injection \\
OTG-INPVAL-014& Testing for Buffer overflow \\

OTG-INPVAL-015& Testing for incubated vulnerabilities \\
OTG-INPVAL-016& Testing for HTTP Splitting/Smuggling \\
OTG-INPVAL-017& Testing for HTTP Incoming Requests \\
OTG-ERR-001& Analysis of Error Codes \\
OTG-ERR-002& Analysis of Stack Traces \\
OTG-CRYPST-001& Testing for Weak SSL/TLS Ciphers, Insufficient Transport Layer Protection \\
OTG-CRYPST-002& Testing for Padding Oracle \\
OTG-CRYPST-003& Testing for Sensitive information sent via unencrypted channels \\
OTG-CRYPST-004& Testing for Weak Encryption \\
OTG-BUSLOGIC-001& Test Business Logic Data Validation \\
OTG-BUSLOGIC-002& Test Ability to Forge Requests \\
OTG-BUSLOGIC-003& Test Integrity Checks \\
OTG-BUSLOGIC-004& Test for Process Timing \\
OTG-BUSLOGIC-005& Test Number of Times a Function Can be Used Limits \\
OTG-BUSLOGIC-006& Testing for the Circumvention of Work Flows \\
OTG-BUSLOGIC-007& Test Defenses Against Application Mis-use \\
OTG-BUSLOGIC-008& Test Upload of Unexpected File Types \\
OTG-BUSLOGIC-009& Test Upload of Malicious Files \\
OTG-CLIENT-001& Testing for DOM based Cross Site Scripting \\
OTG-CLIENT-002& Testing for JavaScript Execution \\
OTG-CLIENT-003& Testing for HTML Injection \\
OTG-CLIENT-004& Testing for Client Side URL Redirect \\
OTG-CLIENT-005& Testing for CSS Injection \\
OTG-CLIENT-006& Testing for Client Side Resource Manipulation \\
OTG-CLIENT-007& Test Cross Origin Resource Sharing \\
OTG-CLIENT-008& Testing for Cross Site Flashing \\
OTG-CLIENT-009& Testing for Clickjacking \\
OTG-CLIENT-010& Testing WebSockets \\
OTG-CLIENT-011& Test Web Messaging \\
OTG-CLIENT-012& Test Local Storage \\
\hline
\end{tabular}

\label{table:OWASPtestingActivities}
\end{table}%


==> tables/tableResults.tex <==
% !TEX root =  ../Main.tex
%\begin{table}[tb]
%%\tiny
%\scriptsize
%%\footnotesize
%\caption{Summary of RQ2 results.}
%%\vspace{-0.25cm}
%\begin{tabular}{|@{\hspace{0.1cm}}p{1.8cm} | @{\hspace{0.05cm}}p{2.0cm} | @{\hspace{0.05cm}}p{3mm} | @{\hspace{0.05cm}}p{3mm} | @{\hspace{0.05cm}}p{3mm} |  @{\hspace{0.05cm}}p{10mm} | @{\hspace{0.05cm}}p{10mm} |  }
%\hline
%\textbf{Case study}&\textbf{Vulnerabilities}&$tp$&$fp$&$fn$&$\mathit{Precision}$&$\mathit{Recall}$\\
%\hline
%\IWS	& 5 & 5& 0& 0 & 1.0 & 1.0\\
%\hline
%Jenkins 2.121.1	& 9 \cite{JV1,JV2,JV3,JV4,JV5,JV6,JV7,JV8,JV9}& \multirow{2}{*}{XX} & \multirow{2}{*}{X} &   \multirow{2}{*}{X}  &   \multirow{2}{*}{X.XX} & \multirow{2}{*}{X.XX}   \\
%Jenkins 2.120& 2 \cite{JV10,JV11}& & & & &\\
%\hline
%\end{tabular}
%%\vspace{-0.5cm}
%\label{table:resultsRQ2}
%\end{table}%





\begin{table}[tb]
%\tiny
\scriptsize
%\footnotesize
\caption{Summary of RQ2 results grouped by data collection method.}
%\vspace{-0.25cm}
\begin{tabular}{|@{\hspace{0.1cm}}p{1.6cm} | @{\hspace{0.05cm}}p{1.5cm} |  @{\hspace{0.05cm}}p{11mm} | @{\hspace{0.05cm}}p{8mm}    |  @{\hspace{0.05cm}}p{11mm} | @{\hspace{0.05cm}}p{8mm} |  }
\hline
\multirow{3}{*}{\textbf{Case study}}&\multirow{3}{*}{\textbf{Vulnerabilities}}&\multicolumn{4}{c|}{\textbf{Data collection method}}\\
&&\multicolumn{2}{c}{\textbf{Crawljax}}&\multicolumn{2}{c|}{\textbf{Crawljax \& Manual}}\\
%\cline{1-2}
&&\textbf{Precision}&\textbf{Recall}&\textbf{Precision}&\textbf{Recall}\\
\hline
\IWS	& 5& 1.0 & 0.80 & 1.0 & 1.0\\
\hline
Jenkins 2.121.1	& \JVulnUsed \cite{JV1,JV2,JV3,JV4,JV5,JV6,JV8,JV9}& 1.0 & 0.50 &   1.0 & 0.75  \\
\hline
\textbf{Overall} & 13 & 1.0 & 0.70 &   1.0 & 0.85  \\
%Jenkins 2.120& 2 \cite{JV10,JV11}& & & & \\
\hline
\end{tabular}
%\vspace{-0.5cm}
\label{table:resultsRQ2}
\end{table}%




%\begin{table}[tb]
%%\tiny
%%\scriptsize
%\footnotesize
%\caption{Oracle problem in OWASP testing activities.}
%%\begin{tabular}{| p{0.07cm} | p{7.8cm} |}
%%\vspace*{-1.2em}
%\begin{tabular}{|c | @{\hspace{0.1cm}}p{3cm} | @{\hspace{0.05cm}}p{1.0cm} |}
%\hline
%&\textbf{Oracle automation strategy}\\
%\hline
%\textbf{Testing activities not }
%&Not required	 &16\\
%\textbf{affected by the oracle} 
%&Single assertion &	9\\
%\textbf{problem.}
%&Implicit oracle	& 4\\
%&Catalog-based	& 11\\
%\hline
%\textbf{Testing activities affected }
%&Manual	& 13\\
%\textbf{by the oracle  problem.}
%&Dedicated methods	& 27\\
%&Metamorphic testing & 17\\
%%TOTAL & 99\\
%\hline
%\end{tabular}
%\vspace*{-1.2em}
%\label{table:OWASPtestingActivities}
%\end{table}%


==> tables/tableVulnerabilityDetails.tex <==
% !TEX root =  ../Main.tex
\begin{table}[tb]
%\tiny
\scriptsize
%\footnotesize
\caption{Discovered vulnerabilities grouped by OWASP ID.}
%\vspace{-0.25cm}
\begin{tabular}{|p{2cm} | p{6mm} | p{18mm} | p{17mm} | }
\hline
\textbf{Vulnerability}&\multicolumn{3}{c|}{\textbf{\# Vulnerabilities Discovered}} \\
&\textbf{IWS}& \textbf{Jenkins 2.121.1} & \textbf{Jenkins 2.120} \\
\hline

OTG-AUTHN-001 &\TENT{1} &  \TENT{-} & \TENT{-} \\
OTG-AUTHN-003 &\TENT{-} &  \TENT{1} & \TENT{-} \\
OTG-AUTHN-004 &\TENT{1} &  \TENT{-} & \TENT{-} \\

OTG-AUTHZ-001&\TENT{1} &  \TENT{3} & \TENT{1} \\
OTG-AUTHZ-002 &\TENT{1} &  \TENT{4} & \TENT{1} \\

OTG-AUTHZ-004&\TENT{1} &  \TENT{-} & \TENT{-} \\
OTG-SESS-003 &\TENT{-} &  \TENT{1} & \TENT{-} \\

\hline
\end{tabular}
\\
\begin{minipage}{8.3cm}
\footnotesize{\textbf{Note}: a dash (-) indicates that the vulnerability does not affect the system.}
\end{minipage}
%\vspace{-0.5cm}
\label{table:resultsRQ2vulns}
\end{table}%



%\begin{table}[tb]
%%\tiny
%%\scriptsize
%\footnotesize
%\caption{Discovered vulnerabilities grouped by OWASP ID.}
%%\vspace{-0.25cm}
%\begin{tabular}{|p{2cm} | p{6mm} | p{8mm} | p{7mm} | p{4mm} |  p{5mm} | p{5mm} |  }
%\hline
%\textbf{Vulnerability}&\multicolumn{3}{c|}{\textbf{\# Vulnerabilities Discovered}}&\multicolumn{3}{|c|}{\textbf{Time before}}\\
%&\textbf{IWS}& \textbf{Jenkins 2.121.1} & \textbf{Jenkins 2.120}&   \multicolumn{3}{|c|}{\textbf{discovery (minutes)}} \\
%&\textbf{IWS}& \textbf{} & \textbf{}& \textbf{min}& \textbf{max} & \textbf{avg}\\
%\hline
%
%OTG-AUTHN-001 &\TENT{1} &  \TENT{-} & \TENT{-} & \TENT{4} &  \TENT{4} & \TENT{4}\\
%OTG-AUTHN-003 &\TENT{-} &  \TENT{1} & \TENT{-} & \TENT{4} &  \TENT{4} & \TENT{4}\\
%OTG-AUTHN-004 &\TENT{1} &  \TENT{-} & \TENT{-} & \TENT{4} &  \TENT{4} & \TENT{4}\\
%
%OTG-AUTHZ-001&\TENT{1} &  \TENT{3} & \TENT{1} & \TENT{4} &  \TENT{4} & \TENT{4}\\
%OTG-AUTHZ-002 &\TENT{1} &  \TENT{4} & \TENT{1} & \TENT{4} &  \TENT{4} & \TENT{4}\\
%
%OTG-AUTHZ-004&\TENT{1} &  \TENT{-} & \TENT{-} & \TENT{4} &  \TENT{4} & \TENT{4}\\
%OTG-SESS-003 &\TENT{-} &  \TENT{1} & \TENT{-} & \TENT{4} &  \TENT{4} & \TENT{4}\\
%
%\hline
%\end{tabular}
%%\vspace{-0.5cm}
%\label{table:resultsRQ2vulns}
%\end{table}%



==> tool.tex <==
\section{Tool Support}
\label{sec:tool}

To ease its industrial adoption, we implemented our approach as a toolset that extends Eclipse IDE~\cite{EclipseIDE}.
%In the following paragraph we provide an overview of the tool. 
Additional information about the toolset, including executable files, download instructions and a screencast covering motivations, are available on the tool's website at \url{https://sntsvv.github.io/SMRL/}. 

Fig.~\ref{fig:toolArchitecture} shows the tool architecture. The main component is the Eclipse plug-in orchestrating the other components in Fig.~\ref{fig:toolArchitecture}. %that
It activates the steps of the approach in Fig.~\ref{fig:approach}.

\begin{figure}[ht]
\centering

\includegraphics[width=0.98\linewidth]{images/architecture_smrl.pdf}

\caption{Tool Architecture}\label{fig:toolArchitecture}

\end{figure}

The components in Fig.~\ref{fig:toolArchitecture} 
automate Steps 1, 2, 3, and 4 in Fig.~\ref{fig:approach}. The \emph{SMRL Editor} supports Step 1 and enables engineers to write new \MRs in \SMRL. It uses Xtext~\cite{Xtext}, a framework for developing programming languages and domain-specific languages, as a third-party component that provides a fully featured, customizable Eclipse-based IDE.

The \textit{Data Collection Framework} automates Step 2 in Fig.~\ref{fig:approach}. As required by Step 4, the \emph{\MT Crawler} systematically browses the system under test to automatically derive source inputs for testing. It takes as input the URL of the system under test and a list of credentials. As discussed in Section~\ref{sec:dataframework}, this component uses and extends the CrawlJax Web crawler~\cite{crawljax:tweb12} as a third-party component. Our extension records additional data (URLs requested by Crawljax actions, data in the HTML forms, and background URL requests), for instance, to replicate modified portions of crawling sessions (see Section~\ref{sec:dataframework}). 

The \emph{SMRL-to-Java Transformer} automatically transforms  \MRs in \SMRL into executable test cases in Java (Step 3 in Fig.~\ref{fig:approach}). To do so, it uses and extends the XBase compiler~\cite{Efftinge2012xbase} that translates the abstract syntax tree of a source specification to Java source code. The \emph{SMRL-to-Java Transformer} takes as input new \MRs written in \SMRL and \MRs selected from our catalog (see Section~\ref{sec:mrs}).

The \emph{\MT Framework} automates Step 4 in Fig.~\ref{fig:approach}. To do so, it implements our \MT algorithm in Section~\ref{sec:mtframework}. The component uses the JUnit test framework~\cite{JUnit} to perform \MT in a traditional testing environment. It takes, as input, executable \MRs in Java and source inputs collected by the \emph{\MT Crawler}.  
